Muffliato: Peer-to-Peer Privacy Amplification for Decentralized Optimization and Averaging

Decentralized optimization is increasingly popular in machine learning for its scalability and efficiency. Intuitively, it should also provide better privacy guarantees, as nodes only observe the messages sent by their neighbors in the network graph. But formalizing and quantifying this gain is challenging: existing results are typically limited to Local Differential Privacy (LDP) guarantees that overlook the advantages of decentralization. In this work, we introduce pairwise network differential privacy, a relaxation of LDP that captures the fact that the privacy leakage from a node $u$ to a node $v$ may depend on their relative position in the graph. We then analyze the combination of local noise injection with (simple or randomized) gossip averaging protocols on fixed and random communication graphs. We also derive a differentially private decentralized optimization algorithm that alternates between local gradient descent steps and gossip averaging. Our results show that our algorithms amplify privacy guarantees as a function of the distance between nodes in the graph, matching the privacy-utility trade-off of the trusted curator, up to factors that explicitly depend on the graph topology. Finally, we illustrate our privacy gains with experiments on synthetic and real-world datasets.

==> app_random_graph.tex <==
The set $\cV$ of nodes (agents) of size $n$ being fixed, let $\cG$ be the set of couples $(G,W)$, where $G$ is a graphw with nodes $\cV$, and $W$ a gossip matrix on $G$. We say that $\cL$ a law over $\cG$ is \emph{node-indistinguishable} if for any $v\in\cV$, conditionally on $\set{v}\cup\cN(v)$ ($\cN(v)$ being the neighbors of node $v$ in the graph sampled from $\cL$), the law of the graph is invariant under any permutation over the set~$\cV\setminus(\set{v}\cup\cN(v))$. We further assume that nodes are only aware on their direct neighbors in the graph; implicitly, this suggests that sampling a graph from $\cL$ is done using only local protocols (Erdös-Rényi graphs, typically). 
In Algorithm~\ref{algo:random-graph-dp-gossip}, a graph is drawn at random, and \textsc{DP-Gossip} (Algorithm~\ref{algo:dp-gossip}) is ran over this graph.

\begin{algorithm}
\KwIn{local values $(x_v)_{v\in\cV}$ to average, a law $\cL$ on $\cG$, number of iterations $T$, noise variance $\sigma^2$}

Sample $(G,W)\sim \cL$

Run \textsc{DP-Gossip}($(x_v)_{v\in\cV},W,T,\sigma^2$) to obtain $x^T_v$ at node $v\in\cV$

\KwOut{$x^T_v$ at node $v\in\cV$}

\caption{\textsc{Random Graph DP-Gossip}($(x_v)_{v\in\cV},\cL,T,\sigma^2)$}
\label{algo:random-graph-dp-gossip}
\end{algorithm}

\begin{theorem}[\textsc{DP-Gossip} on a random graph] Let $\alpha>1$ and $T\geq 0$, $\sigma^2\geq \frac{\alpha(\alpha-1}{2}$ and a law $\cL$ a node-indistinguishable law over $\cG$. Let $u,v\in\cV$ be distinct nodes.
After running Algorithm~\ref{algo:random-graph-dp-gossip} with these parameters, node $u$ is ($\eps_\utov^T(\alpha),\alpha)$-Rényi DP with respect to $v$, with:
\begin{equation*}
    \eps_\utov^T(\alpha)\leq \left\{ \begin{aligned} &\quad\quad\frac{\alpha}{2\sigma^2}\quad\quad \text{ with probability }\proba{\edgeuv\in\cE}\\
    &\frac{\alpha}{\sigma^2} \frac{Td_v}{n-d_v} \quad \text{ with probability }1 -\proba{\edgeuv\in\cE}\end{aligned}\right.\,.
\end{equation*}
The probabilities are taken over the graph $G=(\cV,\cE)$ on the set of nodes $\cV$, sampled from $\cL$.
For an Erdös-Renyi graph of parameters $n,p$ with $p=\frac{cn}{\ln(n)}$ (for $c>1$), $\proba{\edgeuv\in\cE}=p$, the eigengap $\lambda_2$ is of order 1 (so that $T^{\rm stop}=\Tilde\cO(1)$), and $d_v$ is of order $\ln(n)$.
\end{theorem}



\mathieu{Avec randomized ensuite}

\begin{theorem}The iterates $(x^t)_t$ of \textsc{DP-Randomized Gossip} verify, for any $t\geq0$:
\begin{equation*}
    \frac{1}{n}\sum_{v\in\cV}\esp{\NRM{x^t_v-\Bar{x}}^2}\leq\left( \frac{1}{n}\sum_{v\in\cV}\esp{\NRM{x^0_v-\Bar{x}}^2} +\sigma^2\right )e^{-t\lambda_2(p)} + \frac{\sigma^2}{n}\,.
\end{equation*}
\end{theorem}

For $\edgevw\in\cE$ and $T\geq 0$, let $\cP_\edgevw^T=\set{t< T\,:\,\edgevtwt=\edgevw}$. Conditionally on the sequence of edges sampled, we get the following theorem. 

\begin{theorem} After $T$ iterations of \textsc{DP-Randomized Gossip} and conditionally on the edges sampled, node $u\in\cV$ is $(\eps^T_{\utov}(\alpha),\alpha)$-Rényi Differentially private with respect to $v$, with:
\begin{equation*}
    \eps^T_{\utov}(\alpha)\leq \frac{\alpha}{2\sigma^2}\sum_{w\sim v}\sum_{t\in\cP_\edgevw^T}\frac{W(t)_\edgeuw^2}{\NRM{W(t)_w}^2}\,.
\end{equation*}
Taking the mean over $u\in\cV\setminus\set{v}$, we obtain:\mathieu{on s'en fout, dixit edwige, c'est pas très chouette}
\begin{equation*}
    \frac{1}{n}\sum_{u\in\cV\setminus\set{v}}\eps^T_{\utov}(\alpha)\leq \frac{\alpha}{2n\sigma^2} \left|\bigcup_{w\sim v}\cP_\edgevw^T\right|\,.
\end{equation*}
Note that $\left|\bigcup_{w\sim v}\cP_\edgevw^T\right|$ is a discrete Poisson variable of mean $\pi_v T$ where $\pi_v=\sum_{w\sim v}p_\edgevw$.
\end{theorem}
Using this last remark, we can combine randomized communications, with a random graph, just as with synchronous gossip. As before,  node $v$ is only aware of its direct neighbors in graph $G$ drawn at random, and only aware of communications through edges $\edgevw$. Conditionally on $\set{v}\cup\cN(v)$, the law of the graph is invariant under any permutation over the set $\cV\setminus (\set{v}\cup\cN(v))$. 

\begin{cor}[With random graph and random communications] Under these assumptions and if $\sigma^2\geq \frac{\alpha(\alpha-1)}{2}$, we have for any $Z\in\N$:
\begin{equation*}
    \eps_\utov^T\leq \left\{ \begin{aligned} &\quad\quad\frac{\alpha}{2\sigma^2}\quad\quad \text{ with probability }\proba{\edgeuv\in\cE}\\
    &\frac{\alpha}{\sigma^2} \frac{Z}{n-d_v} \quad \text{ with probability }\left(1 -\proba{\edgeuv\in\cE}\right)\times \frac{(\pi_vT)^Z}{Z!}e^{-\pi_v T} \end{aligned}\right.\,.
\end{equation*}
For an Erdös-Renyi graph of parameters $n,p$, with $p=\frac{cn}{\ln(n)}$ (for $c>1$), the eigengap $\bar\lambda_2$ is of order $n$ (so that $T^{\rm stop}=\Tilde\cO(n)$), and $d_v$ is of order $\ln(n)$.

Ne sert pas à grand chose, prendre moyenne pour dire que la formule d'avant amplifie bien, juste en discussion même.
\end{cor}

==> async.tex <==

\section{Private Randomized Gossip}

\edwige{Motivation: flexible, faster, cheaper, fully decentralized
Difficulties: randomization thus worst cases \mathieu{ou alors en proba?}

Algorithm

Utility

Privacy guarantee
}
\mathieu{Ecrire ce qui suit avec du temps continu plutôt ou non? pour la clarté du tout, je préfère ne pas accélérer, mais on peut (et c'est gratuit)}

Randomized gossip consists in adding randomness in communications: for non-negative weights $(p_\edgevw)_{\edgevw\in\cE}$ such that $\sum_{\edgevw\in\cE}p_\edgevw=1$, at iterations $t=0,1,\ldots$
an edge $\edgevtwt\in\cE$ is chosen with probability $p_\edgevtwt$ (independently from the past), and a local averaging is performed \citep{boyd2006randomized}. Denoting $W_\edgevw=I_n-\frac{1}{2}(e_v-e_w)(e_v-e_w)^\top$, this is equivalent to $x^{t+1}=W_\edgevtwt x^t$.
Randomized gossip \citep{boyd2006gossip} is motivated by the flexibility its asynchronous implementation offers, and its fast rate of convergence in terms of number of pairwise communications in the whole graph. We hereby prove that it is also more private than synchronous gossip, by a factor proportional to node degrees. As a consequence, randomized gossip on the complete graph emulates the guarantees of a trusted aggregator, up to logarithmic factors.
We would like to study the utility and DP guarantees of randomized gossip with noisy inputs (\textsc{DP-Randomized Gossip}), namely, the algorithm defined through:
\begin{equation*}
    x^{t+1}=W_\edgevtwt x^t\,,\quad x_v^{0}=x_v+\eta_v\,,
\end{equation*} 
where $(\eta_v)_v$ are \emph{i.i.d.}~centered gaussian of covariance $\sigma^2I_d$.
For $t\geq 0$, we write \begin{equation*}
    W(t)=W_{\set{u_{t-1},v_{t-1}}}\cdots W_{\set{u_0,v_0}}\,,
\end{equation*}
so that $x^t=W(t)x^{0}$.
We also define $\Bar W = \esp{W_\edgevtwt}$ (time independent, since edges are drawn in an \emph{i.i.d.}~fashion). Importantly, notice that $I-\Bar W$ is the Laplacian of graph $G$, with weights $p_\edgeuv$ at edge $\edgeuv$, whose smallest eigenvalue in denoted $\lambda_2(p)$.

\mathieu{corriger notations conflictuelles entre le $p$ du erdos rényi graph, et des intensités d'activations}

 

\begin{theorem}The iterates $(x^t)_t$ of \textsc{DP-Randomized Gossip} verify, for any $t\geq0$:
\begin{equation*}
    \frac{1}{n}\sum_{v\in\cV}\esp{\NRM{x^t_v-\Bar{x}}^2}\leq\left( \frac{1}{n}\sum_{v\in\cV}\esp{\NRM{x^0_v-\Bar{x}}^2} +\sigma^2\right )e^{-t\lambda_2(p)} + \frac{\sigma^2}{n}\,.
\end{equation*}
\end{theorem}

For $\edgevw\in\cE$ and $T\geq 0$, let $\cP_\edgevw^T=\set{t< T\,:\,\edgevtwt=\edgevw}$. The privacy analysis of \textsc{DP-Randomized Gossip} yields the following theorem. The first equation is obtained conditionally on the sequence of edges sampled. In Equation~\ref{eq:double_random_mean}, the mean is taken over the edges sampled and the graph generated. We provide in Appendix~\mathieu{?} a version with exact probabilistic bounds.

\begin{theorem} After $T$ iterations of \textsc{DP-Randomized Gossip} and conditionally on the edges sampled, node $u\in\cV$ is $(\eps^T_{\utov}(\alpha),\alpha)$-Rényi Differentially private with respect to $v$, with:
\begin{equation*}
    \eps^T_{\utov}(\alpha)\leq \frac{\alpha}{2\sigma^2}\sum_{w\sim v}\sum_{t\in\cP_\edgevw^T}\frac{W(t)_\edgeuw^2}{\NRM{W(t)_w}^2}\,.
\end{equation*}
Running \textsc{DP-Randomized Gossip} on an Erdös-Rényi graph with $p=c\frac{\ln(n)}{n}$ for $c>1$ generated as in Algorithm~\ref{algo:ER-dp-gossip} and if $\sigma^2\geq \frac{\alpha(\alpha-1)}{2}$, we have:
\begin{equation}\label{eq:double_random_mean}
    \esp{\eps_\utov^T(\alpha)}\leq \frac{\alpha p}{2\sigma^2} + (1-p) \esp{\frac{2\alpha \pi_v T}{(n-d_v)\sigma^2}}\,,
\end{equation}
where $\pi_v=\sum_{w:\edgevw\in\cE}p_\edgevw$, and $\eps_\utov^T(\alpha)$ concentrates around its mean (Appendix \mathieu{?}).
\end{theorem}
For our choice of $p=c\frac{\ln(n)}{n}$ and for $p_\edgevw=1/|\cE|$, we have $\pi_v=\frac{d_v}{|\cE|}\approx \frac{1}{n}$, and since $d_v$ tightly concentrates around $c\ln(n)$, we have $1/(n-d_v)\sim 1/n$. Consequently, Equation~\ref{eq:double_random_mean} writes as
\begin{equation*}
        \esp{\eps_\utov^T(\alpha)}\leq \cO\left(\frac{\alpha \ln(n)}{2n\sigma^2}+\frac{\alpha \ln(n)T}{2n^2\sigma^2}\right)\,.
\end{equation*}
For our choice of parameters, $\lambda_2(p)$ concentrates around $1/n$, so that the stopping time $T^{\rm stop}$ is of order $n$ (up to logarithmic factors in $n$ and $\sigma^2$), leading to $\esp{\eps_\utov^T(\alpha)}\leq \tilde\cO\left(\frac{\alpha}{2n\sigma^2}\right)$. As a consequence, randomized gossip on an Erdös-Rényi graph emulates the optimal trusted aggregator up to logarithmic factors.

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} We define our relaxation of Local DP formally in Section~\ref{sec:setting}, the gossip averaging is analyzed in Section~\ref{sec:muff} and show substantial amplification, supported by the experiments in Section~\ref{sec:expe}. We define and prove guarantees for decentralized optimization in Section~\ref{sec:gd}.
  \item Did you describe the limitations of your work?
    \answerYes{} We discuss each theorem after in its subsection and show the effective magnitude of the privacy amplification in the experiments (Section~\ref{sec:expe}).
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} We have
included a broader impact statement at the end of the supplementary.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} All our theorems and corollaries have their complete set of assumptions.
	\item Did you include complete proofs of all theoretical results? \answerYes{}, except when proving similar results, we do not repeat the full proof but only explain the main differences. 
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} 
    We provide the code needed to reproduce the results in the supplementary material.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} Most of our experiments have no hyperparameters to tune, and we provide the hyperparameters in Annex for Figure~\ref{fig:gd}.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} see Figures \ref{fig:gd} and \ref{fig:synthe}.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? \answerNo{} All of the simulations ran in a few minutes on a regular laptop.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} We use Houses Dataset and Facebook Ego dataset and cite them.
  \item Did you mention the license of the assets?
    \answerYes{}The dataset Houses is in the public domain, as
indicated on the link provided and the Facebook ego dataset in under BSD license.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}We have included our code in the supplementary.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}



==> syncmean.tex <==

\section{Private Synchronous Gossip}


\mathieu{Introduire une sensitivité !!!} \mathieu{Assumption~\ref{hyp:sensitivity}}

We present our \textsc{DP-Gossip} algorithm: it takes as inputs node values $(x_v)_{v\in\cV}$ to average, a gossip matrix on $G$ and a noise variance $\sigma^2$. Values are initially noised using a Gaussian mechanism, and a Chebychev acceleration of simple synchronous gossip is then used. We formally introduce this algorithm in Algorithm~\ref{algo:dp-gossip} and provide utility guarantees. We then study the individual network differential privacy properties of this algorithms. Throughout the following sections, when studying the averaging problem, we assume that Assumption~\ref{hyp:sensitivity} holds for $\Delta=1$ to ease notations.

\subsection{Private synchronous gossip algorithm and utility analysis}

\begin{algorithm}
\KwIn{local values $(x_v)_{v\in\cV}$ to average, gossip matrix $W$ on a graph $G$, number of iterations $T$, noise variance $\sigma^2$}
$\gamma \leftarrow 2\frac{1-\sqrt{\lambda_W(1-\frac{\lambda_W}{4})}}{(1-\lambda_W/2)^2}$\;
\For{all nodes $v$ in parallel}{
    $x_v^{0} \leftarrow x_v + \eta_v$ where $\eta_v \sim \gau{\sigma^2}$
}
\For{$t = 0$ to $T-1$}{
	\For{all workers $v$ in parallel}{
		\For{all neighbors $w$ defined by $W$}{
			Send $x^t_v$\;
			Receive $x^t_w$\;
		}
		$x^{t+1}_v \leftarrow (1 - \gamma) x^{t-1} + \gamma  \sum_{w \in \mathcal{N}_v } W_{vw} x^t_w$\;
	}
}
\KwOut{$ x_v^T$ at node $v\in\cV$}

\caption{\textsc{DP-Gossip}($(x_v)_{v\in\cV},W,T,\sigma^2)$}
\label{algo:dp-gossip}
\end{algorithm}


The iterates generated by Algorithm~\ref{algo:dp-gossip} write as:
\begin{equation*}
     x^{t}=P_t(W)\big(x^{0}+\gau{\sigma^2I_n}\big)\,,\quad t\geq0\,,
\end{equation*}
where $(P_t)$ is a re-scaled $t^{\rm th}$ Chebychev polynomial (of degree $t$). The utility analysis thus consists in an optimization (or consensus) term vanishing exponentially fast, and a \emph{bias} term due to the initial noisy inputs.
\begin{theorem}[Utility analysis] For any~$T\geq0$, the iterates $(x^T)_{T\geq 0}$ of \textsc{DP-Gossip} (Algorithm~\ref{algo:dp-gossip}) verify:
\begin{equation}\label{eq:dp-gossip-utility}
    \frac{1}{2n}\sum_{v\in\cV}\esp{\NRM{ x^T_v-\Bar{x}}^2}\leq \left( \frac{1}{n}\sum_{v\in\cV}\NRM{x^{0}_v-\Bar{x}}^2 + \sigma^2\right)e^{-T\sqrt{\lambda_W} + \frac{\sigma^2}{n}\,.
\end{equation}
\end{theorem}
There is thus a tradeoff between the variance $\sigma^2$ of the noise initially injected, and the precision reached. For a number of iterations $T^{\rm stop}(W,x,\sigma^2)$ of:
\begin{equation*}
    T^{\rm stop}\big(W,(x_v)_{v\in\cV},\sigma^2\big)=\left\lceil \sqrt{\lambda_W}^{-1}\ln\left(\frac{n}{\sigma^2}\max\left(\sigma^2,\frac{1}{n}\sum_{v\in\cV}\NRM{x^{0}_v-\Bar{x}}^2\right)\right)\right\rceil\,,
\end{equation*}
we have a consensus error $\frac{1}{2n}\sum_{v\in\cV}\esp{\NRM{ x^T_v-\Bar{x}}^2}\leq \frac{3\sigma^2}{n}$, for a minimal number of iterations. This property that is crucial for privacy guarantees and in the utility-privacy tradeoffs we present next.

\subsection{Privacy analysis}


We now turn to the privacy analysis of \textsc{DP-Gossip} (Algorithm~\ref{algo:dp-gossip}), in terms of individual network DP (Definition~\ref{def:indiv_ndp}). Let $\cA^T$ be Algorithm~\ref{algo:dp-gossip} for $T$ steps. In the gossip averaging problem considered, datasets $\cD=(\cD_v)_{v\in\cV}$ correspond to local values: $\cD_v=\set{x_v}$, $v\in\cV$.
The \emph{view} of an agent $v\in\cV$ thus writes as, for any $T\geq1$:
\begin{equation*}
    \cO_v\big(\cA^T(\cD)\big)=\set{\big(W^t(x+\eta)\big)_w\,|\quad \edgevw\in\cE\,,\quad0\leq t\leq T-1}\,,
\end{equation*}
where $\eta\sim\gau{\sigma^2I_{n\times d}}$. We further assume that local values $(x_v)_{v\in\cV}$ lie in a space of diameter $\Delta>0$, that will play the role of \emph{sensitivity}. 

\begin{theorem}[Individual network DP] Let $u,v\in\cV$ be two distinct nodes, $\alpha>0$. After $T$ iterations of \textsc{DP-Gossip} (Algorithm~\ref{algo:dp-gossip}), node $u$ is ($\eps^T_{\utov}(\alpha),\alpha)$ Renyi DP with respect to $v$, with:
\begin{equation}\label{eq:indp}
    \eps^T_{\utov}(\alpha)\leq \frac{\alpha}{2\sigma^2}\sum_{t=0}^{T-1}\sum_{w\sim v}\frac{(W^t)_\edgeuw^2}{\NRM{(W^t)_w}^2}\,.
\end{equation}
This formula can be interpreted in terms of random walks, as:
\begin{equation*}
    \eps^T_{\utov}(\alpha)\leq \frac{\alpha n}{2\sigma^2}\max_{w\sim v}W_\edgevw^{-2}\sum_{t=1}^T\proba{X^t=v|X^0=u}^2\,,
\end{equation*}
where $(X_t)_t$ is the random walk on graph $G$, with transitions $W$.
\end{theorem}

Since expressing pairwise (\emph{i.e.}~between two fixed agents in the graph) utility-privacy tradeoffs using the guarantee offered by~\eqref{eq:indp} would not yield an explicit tradeoff in terms of well-known graph quantities, we formulate the following corollary using the mean formula of Corollary~\ref{cor:mean}, thus making appear the ratio $d_v/\sqrt{\lambda_W}$.

\begin{cor}[Mean formula and privacy-utility tradeoffs]\label{cor:mean}
Let $\eps>0$ and $\alpha>1$.  \textsc{DP-Gossip} after $T$ steps is $(\alpha,f)$-individual network Rényi DP, for $f:\cV\times\cV\to \R^+$ satisfying:
\begin{equation*}
    \frac{1}{n}\sum_{u\in\cV\setminus\set{v}}f(u,v)\leq \eps \,,
\end{equation*}
while having the following utility:
\begin{equation*}
        \frac{1}{2n}\sum_{v\in\cV}\esp{\NRM{ x^{\rm out}_v-\Bar{x}}^2}\leq  \Tilde\cO\left( \frac{d_v}{\eps n^2\sqrt{\lambda_W}}\right)\,,
\end{equation*}
where $x^{\rm out}$ is the output of Algorithm~\ref{algo:dp-gossip} after $T^{\rm stop}(x,W,\sigma^2)$ steps for $\sigma^2=\frac{d_v}{2\alpha\eps}$, $d_v$ is the degree of node $v$, and~$\Tilde\cO$ hides logarithmic factors in $n$ and $\eps$.
\end{cor}

\mathieu{commentaires: ratio $d/\sqrt{\lambda_W}$, ce que ça donne sur quelques graphes: sur ligne et complet, on ne peut pas être plus sharp, sur grille, on est pas mal, sur bons expandeurs c'est super.}


\subsection{Adding graph randomness: the case of Erdös-Rényi graphs}

\mathieu{Erdos renyi}

So far, privacy guarantees come from the initial randomness of noisy inputs. Adding randomness in the graph over which the algorithm is ran and using the same arguments together with the quasi-convexity of Rényi divergences, we show that we can emulate up to logarithmic factors, on networks such as Erdös-Rényi graphs, the privacy guarantees of a trusted aggregator. The random graph assumptions required for our analysis are in fact more general than Erdös-Rényi graphs and presented in Appendix~\mathieu{?}.

We recall that in an Erdös-Rényi graph of parameters $n,p$ over the set of nodes $\cV$ (abbreviated $ER(n,p)$ in the sequel), each edge has a fixed probability $p$ of being present in the graph, independently from the others. Algorithm~\ref{algo:ER-dp-gossip} emulates an Erdös-Rényi graph using local operations, before performing the \textsc{DP-Gossip} algorithm.
We further assume that nodes are only aware on their direct neighbors in the graph, coherent with local communications and the Erdös-Rényi model.


\begin{algorithm}
\KwIn{local values $(x_v)_{v\in\cV}$ to average, parameter $p$, number of iterations $T$, noise variance $\sigma^2$}

Initialize edge set $\cE=\emptyset$

\For{$(v,w)\in\cV^2$ such that $u\ne v$}{
Add $\edgevw$ to $\cE$ with probability $p$
}

Set $W_\edgevw=\frac{1}{\max(d_v,d_w)}$ for $\edgevw\in\cE$.

Run \textsc{DP-Gossip}($(x_v)_{v\in\cV},W,T,\sigma^2$) to obtain $x^T_v$ at node $v\in\cV$

\KwOut{$x^T_v$ at node $v\in\cV$}

\caption{\textsc{Random Graph DP-Gossip}($(x_v)_{v\in\cV},p,T,\sigma^2)$}
\label{algo:ER-dp-gossip}
\end{algorithm}

\begin{theorem}[\textsc{DP-Gossip} on a random graph]\label{thm:privacy-random-graph}
Let $\alpha>1$, $T\geq 0$, $\sigma^2\geq \frac{\alpha(\alpha-1)}{2}$ and $p=c\frac{\ln(n)}{n}$ for $c>1$. Let $u,v\in\cV$ be distinct nodes.
After running Algorithm~\ref{algo:ER-dp-gossip} with these parameters, node $u$ is ($\eps_\utov^T(\alpha),\alpha)$-Rényi DP with respect to $v$, with:
\begin{equation*}
    \eps_\utov^T(\alpha)\leq \left\{ \begin{aligned} &\quad\quad\frac{\alpha}{2\sigma^2}\quad\quad \text{ with probability }\proba{\edgeuv\in\cE}\\
    &\frac{\alpha}{\sigma^2} \frac{Td_v}{n-d_v} \quad \text{ with probability }1 -\proba{\edgeuv\in\cE}\end{aligned}\right.\,.
\end{equation*}
The probabilities are taken over the graph $G=(\cV,\cE)$ on the set of nodes $\cV$.
We have $\proba{\edgeuv\in\cE}=p$, the eigengap $\lambda_W$ is of order 1 \citep{ERgaps2019} (so that $T^{\rm stop}=\Tilde\cO(1)$), and $d_v$ is of order $\ln(n)$.
\end{theorem}

\mathieu{collusions? moyenne aussi?}
